ProPILE: Probing Privacy Leakage in Large Language Models

The rapid advancement and widespread use of large language models (LLMs) have raised significant concerns regarding the potential leakage of personally identifiable information (PII). These models are often trained on vast quantities of web-collected data, which may inadvertently include sensitive personal data. This paper presents ProPILE, a novel probing tool designed to empower data subjects, or the owners of the PII, with awareness of potential PII leakage in LLM-based services. ProPILE lets data subjects formulate prompts based on their own PII to evaluate the level of privacy intrusion in LLMs. We demonstrate its application on the OPT-1.3B model trained on the publicly available Pile dataset. We show how hypothetical data subjects may assess the likelihood of their PII being included in the Pile dataset being revealed. ProPILE can also be leveraged by LLM service providers to effectively evaluate their own levels of PII leakage with more powerful prompts specifically tuned for their in-house models. This tool represents a pioneering step towards empowering the data subjects for their awareness and control over their own data on the web.

==> figure/figure4_likelihood_graphs.tex <==
\begin{figure*}[t!]
    \centering
    \includegraphics[width=\linewidth]{figure/ratio_result.pdf}
    \caption{Number of target PII that can be generated with sampling}
    \label{fig::likelihood_graph}
\end{figure*} 

==> table/dataset.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}\label{table::dataset}
\caption{\small\textbf{Evaluation dataset description.}}
% \vspace{1em}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{rrcc}
\toprule
                              &              & \textbf{Size}           & \textbf{Notes}                                                                                         \\
                              \midrule
\multirow{3}{*}{Structured}   & Twin         & \multirow{3}{*}{10,000} & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Phone number,\\ email address,\\ and address\end{tabular}}\\
                              & Triplet      &                         &                                                                                                       \\
                              % & Quadruplet   &                         &                                                                                                       \\
                        \midrule
\multirow{3.5}{*}{Unstructured} & Relationship & 10,000                  & \begin{tabular}[c]{@{}c@{}}Parents, \\ grandparents, \\ ...\end{tabular}                              \\
\cmidrule{2-4}
                              & Affiliation  & 2,000                   & \begin{tabular}[c]{@{}c@{}}Institution \\ and university\end{tabular}    \\
                            \bottomrule
\end{tabular}
% }
\end{table}
% \vspace{-5pt}

==> table/exact_match_structured.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Perspective of an attacker. Fraction of exactly reconstructed PIIs and edit distances among 50,000 triplets}
\begin{tabular}{cccccc}
\toprule
                       &             & \multirow{2}{*}{Exact match} & \multicolumn{3}{c}{Edit distance}   
                       % & \multicolumn{4}{c}{First-n}                          
                       \\
\cmidrule{4-6} 
                       &             &                              & 1                    & 2                    & 3           
                       % &6 &7 &8 &9 
                       \\
\midrule
\multirow{3}{*}{Phone} & Duplet       &                              &                      &                      &        '
% & & & &             
\\
                       & Triplets    & 71 (0.14\%)         & () 0.27\% & 1.00\% & 1.54\%  
                       % & 178 (3.57\%) & 115 (2.30\%) & 59 (1.18\%) & 13 (0.26\%)
                       \\
                       & Quadruplets &           &   &   &   
                       % &  &  & &  
                       \\
\multirow{3}{*}{Email} & Duplet       &                              &                      &                      &                     
% & & & & 
\\
                       & Triplets    &           &   &   &  
                       % & & & & 
                       \\
                       & Quadruplets &           &   &   &  
                       % & & & &
                       \\
\multirow{3}{*}{Address} & Duplet       &                              &                      &                      &                    
% & & & & 
\\
                       & Triplets    &           &   &   &    
                       % & & & &
                       \\
                       & Quadruplets &           &   &   &    
                       % & & & &
                       \\                       
                       
                       
\bottomrule
\end{tabular}
\end{table}

==> table/reconstruction_likelihood.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Reconstruction likelihood}
\begin{tabular}{ccccccccccccccccc}
\toprule
                                                                         &            & \multicolumn{5}{c}{Reconstruction} & \multicolumn{5}{c}{Null} & \multicolumn{5}{c}{Random} \\
\cmidrule{3-7} \cmidrule{8-12} \cmidrule{13-17}
                                                                         & k-shot     & 1     & 2     & 3    & 4    & 5    & 1   & 2   & 3  & 4  & 5  & 1   & 2   & 3   & 4   & 5  \\
\midrule
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Phone\\ number\end{tabular}}  & Duplet      &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
                                                                         & Triplet    &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
                                                                         & Quadruplet &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
\midrule                                                                         
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Email\\ address\end{tabular}} & Duplet      &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
                                                                         & Triplet    &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
                                                                         & Quadruplet &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
\midrule
\multirow{3}{*}{Address}                                                 & Duplet      &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
                                                                         & Triplet    &       &       &      &      &      &     &     &    &    &    &     &     &     &     &    \\
                                                                         & Quadruplet &       &       &      &      &      &     &     &    &    &    &     &     &     &     &   \\
\bottomrule
\end{tabular}
\end{table}

==> table/reconstruction_likelihood_unstructured.tex <==
\begin{table}[]
\centering
\caption{Perspective of attackers}
\begin{tabular}{cccc}
\toprule
             & Reconstruction & Null & Exact match  \\
\midrule
Relationship &                &      &  \\
Institution  &                &      &  \\
\bottomrule
\end{tabular}
\end{table}

==> table/soft_embedding.tex <==
% \begin{table}[]
% \centering
% \caption{}
% \begin{tabular}{ccccc}
% \toprule
%             & \multicolumn{4}{c}{w/ soft prompt} 
%       &      & w/o soft prompt & N_\mathrm{train}=16 & w/o soft prompt & w/ soft prompt\\
% \midrule
% \textbf{Likelihood}  &   5.46e-08                 &  5.82e-05             & &    \\
% \textbf{Exact match} &   0.11\%                & 1.28\%                & & \\
% \bottomrule
% \end{tabular}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}


%%%%%%%% Version 2# %%%%%%%%%%
% \begin{table}[]
% \centering
% \caption{White-box probing result.}
% \begin{tabular}{cccccccc}
% \toprule
%             & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{w/o} \\ \textbf{soft prompt}\end{tabular}} & \multicolumn{6}{c}{\textbf{w/ soft prompt}}\\
%             \cmidrule{3-8}
%             &                                  & $N\!=\!16$ & $N\!=\!32$ & $N\!=\!64$ & $N\!=\!128$ & $N\!=\!256$ & $N\!=\!512$ \\
% \midrule
            
% Likelihood  &                                  &               &               &               &                &                &                \\
% Exact match (\%) &                                  &               &               &               &                &                & \\

% \multicolumn{1}{l}{} & \multicolumn{1}{l}{}                                                        & $N\!=\!128$        & $N\!=\!128$        & $N\!=\!128$        \\
% Likelihood           & \multicolumn{1}{l}{}                                                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} \\
% Exact match          & \multicolumn{1}{l}{}                                                        & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{}

% \bottomrule
% \end{tabular}
% \end{table}


% \begin{table}[]\label{table::soft_prompt}
% \centering
% \caption{White-box probing result.}
% \begin{tabular}{ccccc}
% \toprule
%             & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{w/o} \\ \textbf{soft prompt}\end{tabular}} & \multicolumn{3}{c}{\textbf{w/ soft prompt}}\\
%             \cmidrule{3-5}
%             &                                  & $N\!=\!16$ & $N\!=\!32$ & $N\!=\!64$  \\
% \midrule
            
% Likelihood  &                                  &               &               &                            \\
% Exact match (\%) &                                  & $0.12 \pm $             & $0.31 \pm $               & $0.53 \pm $            \\
% \midrule
% \multicolumn{1}{c}{} & \multicolumn{1}{c}{}                                                        & $N\!=\!128$ & $N\!=\!256$ & $N\!=\!512$        \\
% \cmidrule{3-5}
% Likelihood           & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\
% Exact match (\%)          & \multicolumn{1}{c}{}                                                        & \multicolumn{1}{c}{} & \multicolumn{1}{c}{$\textbf{1.99}\pm0.17$} & \multicolumn{1}{c}{$1.34\pm$  }
% \\
% \bottomrule
% \end{tabular}
% \end{table}

\begin{table}[]\label{table::soft_prompt}
\centering
\resizebox{0.6\columnwidth}{!}{
\caption{White-box probing result.}
\begin{tabular}{ccccc}
\toprule
            & \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{w/o} \\ \textbf{soft prompt}\end{tabular}} & \multicolumn{3}{c}{\textbf{w/ soft prompt}}\\
            \cmidrule{3-5}
            &                                  & $N\!=\!16$ & $N\!=\!32$ & $N\!=\!64$  \\
\midrule
            
Likelihood  & $2.71\!\times\!10^{-8}$                                 &  $1.68\!\times\!10^{-5}$            &  $1.76\!\times\!10^{-4}$             &  $1.81\!\times\!10^{-4}$                          \\
Exact match (\%) &  $0.019$                                & $0.12 \pm $             & $0.31 \pm $               & $0.53 \pm $            \\
\midrule
& \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{w/o} \\ \textbf{soft prompt}\end{tabular}} & \multicolumn{3}{c}{\textbf{w/ soft prompt}}\\
            \cmidrule{3-5}
            &                                  & $N\!=\!128$ & $N\!=\!256$ & $N\!=\!512$  \\
\midrule
Likelihood  &    $2.71\!\times\!10^{-8}$                              & $2.86\!\times\!10^{-4}$               & $4.21\!\times\!10^{-4}$              &   $2.54\!\times\!10^{-4}$                         \\
Exact match (\%) &  $0.019$                              & $1.50 \pm $             & $1.38\pm $               & $1.41 \pm $            \\
\bottomrule
\end{tabular}
}
\end{table}


==> table/soft_embedding_transfer.tex <==
\begin{table}[]\label{table::transfer}
\centering
\captionsetup{font=small}
\caption{\textbf{Transferability of soft prompt}. 
% The soft prompt learned from a source model is projected to hard tokens and then feed forwarded to the target model. 
% All results are from probing target models. 
Original denotes the black-box probing results and transfer denotes the probing results using the soft prompt learned from the source model (OPT-1.3B). 
$\times$ columns shows how much the leakage likelihood increases by using the transferred soft prompt.
}
\begin{adjustbox}{width=0.8\columnwidth,center}
\begin{tabular}{ll|ccc|cc}
\toprule
\textbf{Source}       &\textbf{Target}          & \multicolumn{3}{c|}{\textbf{Likelihood} } & \multicolumn{2}{c}{\textbf{Exact match}} \\
% & \textbf{\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\textbf{Projection} \\ \textbf{error}\end{tabular}}}\\
% \cmidrule{3-4} \cmidrule{5-6}
% \midrule
  &      & Original       & Transfer  & $\times$     & Original       & Transfer       \\
\midrule
\multirow{2}{*}{\texttt{OPT-1.3B}} & \texttt{OPT-350M}   & $1.05\!\times\! 10^{-11}$                &   $1.08\!\times\!10^{-10}$      & \textbf{7.5}      &   0             & 0                \\
& \texttt{OPT-1.3B} & $6.06\!\times\!10^{-8}$               & $3.47\!\times\!10^{-6}$        & \textbf{57.3}      & 5          & 3 \\
 & \texttt{OPT-2.7B} & $1.39\!\times\!10^{-7}$               & $2.18\!\times\!10^{-6}$         & \textbf{15.6}    &  14         & 15 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\end{table}

==> texts/1.Introduction.tex <==
Recent years have seen staggering advances in large language models (LLMs)~\cite{radford2019language, brown2020language, thoppilan2022lamda, chowdhery2022palm, scao2022bloom, touvron2023llama, openai2023gpt4}.
The remarkable improvement is commonly attributed to massive scale training data crawled extensively from the web.




With their outstanding capabilities in language understanding, an explosive number of users shortly began to use the related services, e.g., ChatGPT reached 100 million monthly users in two months after its launching. 
The remarkable improvement is commonly attributed to extensively learning large-scale web-crawled documents produced by the massive general public. 
Data subject

But the dependency on web-crawled datasets raised various ethical concerns such as harmful content generation, hallucinations, and fake content generation~\cite{bang2023multitask, ji2023survey, bommasani2021opportunities}.

Recent findings suggests that LLMs \textit{memorize} texts in training dataset~\cite{feldman2020neural, inan2021training, carlini2022quantifying}. 
It is true that not all memorizations are problematic. 
In fact, LLM should memorize training examples to some extent to improve the utilities.
For example, the structure of sentences, correspondence between words, or common idioms are the things that should be memorized to improve the quality of the generated sentences. 
However, the surprising fact has been reported that about 1\% of datasets are \textit{verbatim} generated given the prefix~\cite{carlini2021extracting}.

This finding raises serious concerns, especially about private data leakage~\cite{carlini2021extracting, carlini2022quantifying, huang2022large, lukas2023analyzing}. 
Web-collected training dataset for LLMs contain sensitive personal information crawled from the personal web pages, social media accounts, personal profiles in online forums, and online databases such as collections of in-house emails~\cite{huang2022large}. 
Such personal information includes the subjects' names, phone numbers, addresses, university they graduated from, family members, religion, a political inclinations, to name a few. 
Serious privacy leakage takes place when certain prompts induce the generation of such information to ``any'' LLM user, not necessarily the data subject.
The scale of potential privacy leakage for LLM is hardly matched by any previous web services: LLMs are used by massive number of users worldwide and they have essentially equal access to such private information. 

Considering that the training dataset is collected from web, this implies that once your personal private information is posted online, it can be potentially included in the training dataset of an LLM, and then might be getting silently leaked from it.
This leakage may cause harm to an unspecified majority. 
As soon as possible before LLMs are used in a wider range of social applications, individual users should be provided with a tool to probe if their data are being leaked by LLMs, and also service providers should inspect whether their services are violating privacy regulations by memorizing the private information.
Despite this urgency, there has been no attempt to establish such probing schemes.

% Not all memorization is problematic. 
% Indeed, it is obvious that LLM memorizes part of training dataset to improve utilities.
% The structure of sentences, the correspondence between words, or common idioms are the thing that should be memorized to guarantee the quality of the generated sentences. 
% However, what if your PII is memorized and generated from the LLMs? 
% This leakage may serve as a big threat on various LLM usages. 

In this paper, we propose to probe PII leakage in LLM which can help users to investigate how likely their own PII is leaked from LLMs.
In particular, we first propose to comprehensively formulate PII according to its associativity and the linguistic structurality.
Then we introduce two probing scenarios, black-box and white-box, according to the user's objective and capability.
Under the two scenarios, we propose probing strategies based on prompting and soft prompt tuning.
We also introduce two categories of metrics that quantify the leakage in diverse perspectives. 

Using these strategies, we conduct actual probing of various existing LLMs with carefully designed evaluation dataset and report valuable findings that need to be noticed by service users and providers.
Our empirical findings using prompting show that a surprising amount of PII is reconstructed from LLMs even with simple, hand-crafted prompts more than expected.
Even if the PII is not leaked with few manually crafted prompts, we show that it still can be exposed with learned soft prompts.
We expect that our formulation and observation serves as a strong incentive for both users and LLM service provider to raise awareness and demand for privacy protection. 
% how much private data is being leaked from open source language model and also report that unexpectedly high leakage probability with learned prompts.
% We believe that our work help users to probe potential misuse 

% \begin{itemize}
%     % \item LLM explodes but there are lots of concern on its trustworthiness - Recent LLMs are trained with web-crawled data which may include our own private information (Twitter case?). Italy even bans the use of ChatGPT.
%     % \item Even your own data may be included in the training data of such large language models without your knowledge. If the LLM never leaks the information, then it is not a big problem. However, do you really think that LLM keeps the secret? Surprisingly, it does not. Rather it leaks more information than you think.
%     % \item LLM memorizes training data, previous works especially warn the privacy issue of personal identifiable information being extracted. 
%     % \item Limitations of previous works on memorization: 1) only prefixes retrieved from the training data have been tested (Conventional generate-and-evaluate approach, where the sentences are generated given prefixes and the generated suffices are compared to the texts in training dataset.) 2) only few PIIs have been tested - in order to use the exploded LLMs with trust, we should thoroughly examine how likely it is that PIIs will leak from LLM.
%     % \item Naive filtering or rule-based filtering system may fail because soft prompt that might seem unsensical to human can result in significant amount of leakage. 
%     % \item PII leakage becomes severe problem when it is extracted within the context. (Association). Unlike the common belief that LLM cannot perform well in the association cases, we found that PIIs are leaked more frequently than was believed.
%     % \item LLM secretly reveals your private information - soft prompt tuning will increase the likelihood of PII being reconstructed.
%     % Unlike the conventional approach, this poses more concern on the privacy issue since this indicates that an attacker may succeed the attack even if he/she manually construct the prompt with partially known personal information.
%     \item Contributions
% \end{itemize}



% \input{figure/figure1_text_example}

